Unbiased Approximate Vector-Jacobian Products for Efficient Backpropagation

In this work we introduce methods to reduce the computational and memory costs of training deep neural networks. Our approach consists in replacing exact vector-jacobian products by randomized, unbiased approximations thereof during backpropagation. We provide a theoretical analysis of the trade-off between the number of epochs needed to achieve a target precision and the cost reduction for each epoch. We then identify specific unbiased estimates of vector-jacobian products for which we establish desirable optimality properties of minimal variance under sparsity constraints. Finally we provide in-depth experiments on multi-layer perceptrons, BagNets and Visual Transfomers architectures. These validate our theoretical results, and confirm the potential of our proposed unbiased randomized backpropagation approach for reducing the cost of deep learning.

==> figures_tex/all_methods_grid.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_diag_optimal}
        \caption{corr\_diag\_optimal}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_diag_optimal_sec_mom}
        \caption{corr\_diag\_optimal\_sec\_mom}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_optimal}
        \caption{corr\_optimal}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_optimal_sec_mom}
        \caption{corr\_optimal\_sec\_mom}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_svd_topr}
        \caption{corr\_svd\_topr}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_svd_topr_squared}
        \caption{corr\_svd\_topr\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_topr_l1}
        \caption{corr\_topr\_l1}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_topr_l1_squared}
        \caption{corr\_topr\_l1\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_topr_l2}
        \caption{corr\_topr\_l2}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_topr_l2_squared}
        \caption{corr\_topr\_l2\_squared}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_topr_var}
        \caption{corr\_topr\_var}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/corr_topr_var_squared}
        \caption{corr\_topr\_var\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/diag_optimal}
        \caption{Diag optimal}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/diag_optimal_sec_mom}
        \caption{diag\_optimal\_sec\_mom}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/ew_sparse_jac}
        \caption{Element-wise Masking}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/optimal}
        \caption{Optimal}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/optimal_sec_mom}
        \caption{optimal\_sec\_mom}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/partial_participation}
        \caption{Partial Participation}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/svd_topr}
        \caption{SVD top-r}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/svd_topr_squared}
        \caption{svd\_topr\_squared}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/topr_l1}
        \caption{topr\_l1}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/topr_l1_squared}
        \caption{topr\_l1\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/topr_l2}
        \caption{$\ell_2$-top r}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/topr_l2_squared}
        \caption{topr\_l2\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_all/topr_var}
        \caption{var-top r}
    \end{subfigure}

    \pgfplotslegendfromname{sharedlegend}

    \caption{Best accuracy reached by the different methods when $p$ varies.}
    \label{fig:all_methods_grid}
\end{figure*}


==> figures_tex/mlp_all.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_svd_topr}
        \caption{corr\_svd\_topr}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_svd_topr_squared}
        \caption{corr\_svd\_topr\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_topr_l1}
        \caption{corr\_topr\_l1}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_topr_l1_squared}
        \caption{corr\_topr\_l1\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_topr_l2}
        \caption{corr\_topr\_l2}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_topr_l2_squared}
        \caption{corr\_topr\_l2\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_topr_var}
        \caption{corr\_topr\_var}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/corr_topr_var_squared}
        \caption{corr\_topr\_var\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/diag_optimal}
        \caption{Diag optimal}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/ew_sparse_jac}
        \caption{Element-wise Masking}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/optimal}
        \caption{Optimal}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/partial_participation}
        \caption{Partial Participation}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/svd_topr}
        \caption{SVD top-r}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/svd_topr_squared}
        \caption{svd\_topr\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/topr_l1}
        \caption{topr\_l1}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/topr_l1_squared}
        \caption{topr\_l1\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/topr_l2}
        \caption{$\ell_2$-top r}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/topr_l2_squared}
        \caption{topr\_l2\_squared}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/topr_var}
        \caption{var-top r}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/topr_var_squared}
        \caption{topr\_var\_squared}
    \end{subfigure}

    \vspace{0.25cm}

    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \tikzfig[\textwidth]{figures_tex/mlp_method_wise/uniform}
        \caption{Uniform Sketching}
    \end{subfigure}

    \pgfplotslegendfromname{sharedlegend}

    \caption{Best accuracy reached by the different methods when $p$ varies.}
    \label{fig:all_methods_grid}
\end{figure*}

